Symmetric Graph Convolutional Autoencoder for Unsupervised Graph Representation Learning

We propose a symmetric graph convolutional autoencoder which produces a low-dimensional latent representation from a graph. In contrast to the existing graph autoencoders with asymmetric decoder parts, the proposed autoencoder has a newly designed decoder which builds a completely symmetric autoencoder form. For the reconstruction of node features, the decoder is designed based on Laplacian sharpening as the counterpart of Laplacian smoothing of the encoder, which allows utilizing the graph structure in the whole processes of the proposed autoencoder architecture. In order to prevent the numerical instability of the network caused by the Laplacian sharpening introduction, we further propose a new numerically stable form of the Laplacian sharpening by incorporating the signed graphs. In addition, a new cost function which finds a latent representation and a latent affinity matrix simultaneously is devised to boost the performance of image clustering tasks. The experimental results on clustering, link prediction and visualization tasks strongly support that the proposed model is stable and outperforms various state-of-the-art algorithms.

==> 1-Introduction_HJ.tex <==
\section{Introduction}

%%%%%%%%%%%%%%%%%%
\input{figure_1}
%%%%%%%%%%%%%%%%%%

A graph, which consists of a set of nodes and edges, is a powerful tool to represent the geometric structure of data. 
There are various applications using graphs in machine learning and data mining researches such as node clustering \cite{ng2002spectral}, dimensionality reduction \cite{belkin2002laplacian}, social network analysis \cite{lazer2009life}, chemical property prediction of a molecular graph \cite{duvenaud2015convolutional}, \jw{and image segmentation \cite{shi2000normalized}}. \hj{It would be great if we list at least one computer vision application.}
% However, conventional graph analyzing methods have several problems like low computational efficiency due to eigendecomposition or singular value decomposition, or showing the only shallow relationship between nodes since it is hard to apply as an input of a deep neural network model.
% \jw{새로운 흐름: 1. 기존 방법 구조의 문제점 2. 새로운 구조의 필요 대두(어떤 구조가 필요한지 적기) 3. 새로운 구조를 위해 laplacian sharpening이 필요함. 4. 필요한 것을 안정성있게 하기 위해, 그리고 클러스터링을 잘 하기 위해 이런저런 것을 추가하였다.}
In recent years, there is an emerging field called \textit{geometric deep learning} \cite{bronstein2017geometric}, which generalizes deep neural network models to non-Euclidean domains such as meshes, manifolds, and graphs. 
The geometric deep learning enables us to learn a deep representation of the geometric structure of a graph \cite{kipf2017semi,monti2017geometric,litany2017deformable}.
Among them, finding deep latent representations of the geometrical structures of graphs using an autoencoder framework is getting growing attention.
In this paper we focus on the node clustering task of the graph data in an unsupervised manner by using the autoencoder framework based graph convolutional network. 

There have been several autoencoder based GCN \cite{kipf2016variational, pan2018adversarially, wang2017mgae} which encode latent representation of the graphs.
However the conventional graph convolutional autoencoder algorithms do not fully utilize the graph structure information and node features in the decoder part due to their incomplete structures, which is limited to finding better latent representations.

Furthermore, to increase the performance of graph data clustering, there are several algorithms \cite{yang2017towards}, \cite{ji2017deep}, \cite{yang2017graph} which show the superior clustering performance by adding clustering cost function like k-mean clustering, spectral clustering or subspace clustering \cite{vidal2011subspace} on the deep neural network cost to make the clustering-friendly latent representations. However, if there are $n$ data points, their algorithm requires at least $n^2$ parameters to seek self-expressive latent representations. This limits the range of applications to small datasets only.

In this paper, we propose a novel graph convolutional autoencoder framework which has complete symmetric autoencoder architecture and uses both the structure of the graph and node attributes in both the encoding and decoding processes. 
Our design of the decoder part is motivated from the analysis in a recent paper \cite{li2018deeper}, that the encoder of 
VGAE \cite{kipf2016variational} can be interpreted as a special form of Laplacian smoothing \cite{taubin1995signal} that computes the new representation of each node as a weighted local average of neighbors and itself. 
By doing so, the features in the same cluster become similar, which makes clustering much easier and improves the performances.
This interpretation has inspired us to design %consider 
a decoder as \emph{Laplacian sharpening}, which is a counterpart of Laplacian smoothing.
% As a result, the decoder can make %, which makes 
% each node farther away from the centroid of its neighbors, which might be actually good for the purpose of input sample reconstruction.
Also, since Laplacian sharpening can decode the latent representation by using both the graph structure and node features, our enhanced decoder can find a better latent representation that reflects the structure of the graph more clearly.
In addition, to increase the clustering performance, we merged the subspace clustering cost function \cite{ji2017deep} into the reconstruction cost of the autoencoder, and in order to make our algorithm capable of handling large-scale datasets, we derive a computationally efficient cost function for the clustering-friendly latent representation.

The main contributions of this paper can be summarized as follows: 
\begin{itemize}
\item The first complete graph convolutional autoencoder architecture in which both of the encoding and decoding processes can utilize the structure of the graph and node attributes concurrently. 
\item A new numerically stable form of decoder preventing the numerical instability of the network
\item A new cost function that can impose the clustering-friendly latent space with reducing the computational burdens.
\end{itemize}

In experiments, our proposed framework is validated by comparing it with the state-of-the-art methods and visualizing the graph clustered by our framework, and our framework shows superior clustering performance on the graph data among several graph-based clustering algorithms. 

==> 2-Related_Works.tex <==
\section{Related Works}

\noindent\textbf{Autoencoder based GCN: }
The first attempt is VGAE \cite{kipf2016variational} which consists of a graph convolutional network (GCN) \cite{kipf2017semi} encoder and a matrix inner-product decoder \jw{as shown in Figure \ref{comparison}. (a)}. % based on variational autoencoder (VAE) \cite{kingma2013auto}.
VGAE has been applied to link prediction task and has shown competitive results.
%After the success of VGAE, the variants of VGAE have been proposed. 
As a variant of VGAE, ARVGA \cite{pan2018adversarially} has been proposed by adding adversarial approaches to VGAE.
However, VGAE and ARVGA use topological structures of the graph only in the encoder part to find the latent representation. 
Since the latent representation was found by the encoder using a topological structure of graphs, it is natural that the reconstructed representation also calculated by the decoder utilizing the information of graphs.
\jw{In addition, since the decoder part cannot be learnable, finding the meaningful latent representation is solely dependent on the learning the weights of the encoder part.
And, although the goal of VGAE and ARVGA is to restore the structure of the graph (i.e. affinity matrix), the information about graph does not used at all in the decoder part. 
These facts can degrade the capability of graph learning.}
Then, MGAE \cite{wang2017mgae} has been proposed, which uses stacked single layer graph autoencoder with linear activation function and marginalization process \jw{as shown in Figure \ref{comparison}. (b)}.
However, MGAE reconstructs the feature matrix of nodes without hidden layers,
%using single layer structure, 
they cannot attain low-dimensional latent representations, which is not complete autoencoder form.
\jw{Also, since MGAE cannot manipulate the dimension of the latent representation and uses linear activation function, there is a distinct limit to finding latent representations in which the structure of the graph is clearly revealed.}

==> figure_4.tex <==
\begin{figure*}[h!]
\centering
% \vspace{0.5cm}
\begin{subfigure}{.245\textwidth}
\centering
\includegraphics[clip, trim = 2.8cm 0.3cm 2.2cm 0.1cm, width=0.95\linewidth]{figure/coil20_original_dot.png}
\caption{COIL20 (raw node feature) \\ \textcolor{white}{f} \hspace{0.3cm}}
\end{subfigure}
\begin{subfigure}{.245\textwidth}
\centering
\includegraphics[clip, trim = 2.8cm 0.9cm 2.2cm 0.1cm, width=0.95\linewidth]{figure/coil20_coco_dot.png}
\caption{COIL20 (result of GALA) \\ \textcolor{white}{f} \hspace{0.3cm}}
\end{subfigure}
\begin{subfigure}{.245\textwidth}
\centering
\includegraphics[clip, trim = 4cm 1.8cm 4cm 1.4cm, width=0.95\linewidth]{figure/yale_original_dot.png}
\caption{YALE (raw node feature) \\ \textcolor{white}{f} \hspace{0.3cm}}
\end{subfigure}\hfill
\begin{subfigure}{.245\textwidth}
\centering
\includegraphics[clip, trim = 4cm 1.8cm 4cm 1.4cm, width=0.95\linewidth]{figure/yale_coco_dot.png}
\caption{YALE (result of GALA) \\ \textcolor{white}{f} \hspace{0.3cm}}
\end{subfigure}\hfill
\caption{
The two-dimensional visualizations of features of each node and the latent representations of GALA for COIL20 and YALE are presented.
The projection is conducted by t-SNE.
The same color indicates the same cluster.
}
\label{visualization_image}
\end{figure*}

==> table_6.tex <==
\begin{table}[t]
\caption{Test time analysis (\textit{sec})}
\footnotesize
\begin{tabu}{c | X[c] | X[c] | X[c]}
\toprule[1pt]
& Cora & Citeseer & Wiki \\
\midrule
Messy loss (Eq. \ref{messy_loss}) & 15.74 & 25.46 & 16.58 \\
Efficient loss (Eq. \ref{final_loss}) & \textbf{13.54} & \textbf{20.34} & \textbf{14.22} \\
\bottomrule[1pt]
\end{tabu}
\label{time}
\end{table}
